ChemReasoner: Heuristic Search over a Large Language Model's Knowledge Space using Quantum-Chemical Feedback

The discovery of new catalysts is essential for the design of new and more efficient chemical processes in order to transition to a sustainable future. We introduce an AI-guided computational screening framework unifying linguistic reasoning with quantum-chemistry based feedback from 3D atomistic representations. Our approach formulates catalyst discovery as an uncertain environment where an agent actively searches for highly effective catalysts via the iterative combination of large language model (LLM)-derived hypotheses and atomistic graph neural network (GNN)-derived feedback. Identified catalysts in intermediate search steps undergo structural evaluation based on spatial orientation, reaction pathways, and stability. Scoring functions based on adsorption energies and reaction energy barriers steer the exploration in the LLM's knowledge space toward energetically favorable, high-efficiency catalysts. We introduce planning methods that automatically guide the exploration without human input, providing competitive performance against expert-enumerated chemical descriptor-based implementations. By integrating language-guided reasoning with computational chemistry feedback, our work pioneers AI-accelerated, trustworthy catalyst discovery.

==> iclr2024-latex/4.5discussion.tex <==


\section{Discussion}








==> iclr2024-latex/4results_consistency.tex <==

%\subsection{Coherency in Reasoning Pathways}

%\carl{Discuss the embedding-based coherency metric here. Also do a little qualitative analysis. }


%\carl{(RQ2)}




==> iclr2024-latex/4results_qualitative.tex <==
\subsection{Qualitative Evaluation}

==> iclr2024-latex/4results_towards.tex <==

%\subsection{Towards Explainable Reasoning from Chemical Feedback}



==> iclr2024-latex/6limitations.tex <==


\section*{Limitations}

In this work, we consider applications of large language models in the scientific domain. In general, this comes with a number of limitations. First, LLMs display largely black box behavior, which is exacerbated by many strong models only being accessible as APIs. Second, generative modeling in the scientific domain is incredibly difficult to evaluate, requiring laboratory verification in many settings. Third, hallucination about factual information is a concern. One benefit of our method is that it provides reasonings based on refined prompts, which we show can be inspirational to domain experts searching for a solution. 
In particular, our reward function based on LLM outputs of scientific questions can be considered a limitation. However, it allows for much quicker validation of ideas and we find it to be an effective proxy (which on its own is interesting). In the future, comparatively costly atomistic simulations can be used to replace our reward function. These can be quite time-consuming and computationally expensive, so we focus on our algorithmic contribution in this work.  % and would significantly increase compute requirements and query latency. 
% can be used in the MCR algorithm. 
Because of the efficacy we demonstrate using LLM rewards, it may also be possible to use a hybrid approach to save on computational chemistry simulations. This could initially leverage LLM embeddings as an reward to narrow down promising search subtrees by selecting the most promising nodes in the first few layers of the search tree. Advanced simulations can then be used for searching final answers in these subtrees. Alternatively, simulations can be used as a limited-use oracle like in active learning. We leave this for future work. 

Our method's improvement comes with higher cost of inference, similar to Tree-of-Thought. When doing inference locally, this may not be a problem. However, we utilize third-party APIs which are both expensive and rate-limited. We found existing open-source models trained on chemistry text did not possess sufficient instruction-following capabilities to be reliable or effective here. Thus, we were limited in quantity of experiments that could be done, as well as the models which could be accessed. This is because our approach requires an average of 750 API calls per tree search. Although this is a limitation of our experiment, we achieve 25.8\% better results than BFS. Although we evaluate on relatively few initial questions, our in-depth expert-performed analysis is based on $\sim$7,200 queries.


\section*{Ethical Considerations}
We propose a zero-shot prompting methodology for LLMs that enables reasoning for complex queries in the scientific domain. Like most applications of LLMs, this has similar ethical considerations, especially in regards to implicit biases from large-scale pretraining and the hallucination of false information. Thus, it is still important for human oversight and careful evaluation of language model output. One consideration of our method is that it may enable discovery of molecules, materials, or other scientific products which can be used for harmful applications \cite{urbina2022dual}. Overall, we believe these downsides are outweighed by the benefits of this work to both the NLP community and other scientific communities which may benefit.


==> iclr2024-latex/backup/introduction.tex <==

\section{Introduction}

The discovery of optimal factor combinations that maximize desired properties drives empirical fields such as chemistry. Chemists actively reason to mentally search through reactants, catalysts, and operating conditions that could enable more efficient chemical conversions demanding less energy. As proposed by seminal work on descriptor-based catalyst search \cite{norskov2011density}, linking microscopic surface properties to macroscopic catalytic performance via chemical descriptors (or properties) is key to accelerating such hypothesis generation.

large language models (LLMs) \cite{wei2022chain, ouyang2022training, taylor2022galactica, BiomedicalLM2023, openai2023gpt4} now bring within reach the realization of such data-driven autonomous search to accelerate scientific discovery. However, concerns around sensitivity to prompts and hallucination remain \cite{creswell2022faithful, taylor2022galactica}.  



Scientific discovery thrives on uncovering the optimal combinations of factors that maximize a property of interest. For highly empirical fields such as chemistry, such combinatorial searches coupled with scientific reasoning is mentally performed by practitioners for hypothesis generation. For example, to discover new energy efficient fuels \cite{yang2019machine, tran2023open, zitnick2020introduction} or efficient chemical conversion processes requiring less energy, a scientist would need to consider the chemical reaction, the reactants that undergo the reaction, the catalysts that improve the rate of reaction, and find the optimal combination of operating conditions (Fig. \ref{fig:challenge_and_approach}).  The seminal work by \cite{norskov2011density} introduced the vision for descriptor-based search for catalysts proposed where microscopic surface properties are linked to macroscopic catalytic properties via selected chemical descriptors (or properties). The original paper expressed the vision for searching over a hypothetical database that stored performance metrics for any group of chemical descriptors.  Promising candidates returned by such a search would be further screened by computational chemistry simulations and experiments in the laboratory.
The emerging capability of large language models (LLMs) \cite{wei2022chain, ouyang2022training, taylor2022galactica, BiomedicalLM2023, openai2023gpt4} provides an opportunity to realize such vision via autonomous machine reasoning and accelerate scientific discovery.  Despite their promise, the sensitivity of language models to their inputs and hallucination remain areas for concern \cite{creswell2022faithful, taylor2022galactica}. In addition to addressing these challenges, providing answers with high specificity using key technical terminology (Fig. \ref{fig:challenge_and_approach}) is essential to earn the scientific community's trust and pave the way for adoption of machine reasoning systems. 

\begin{figure*}[h]
  \centering
  \includegraphics[width=1.0\textwidth]{iclr2024-latex/figures/approach.png}
\caption{ChemReasoner successively ``thinks in terms of" different constraints and factors, each of which are related via scientific principles, and narrow down the set of possible candidates.  It accomplishes that by prompting a language model with different combinations, yielding a tree-structured space of queries and potential candidates, and returns the optimal answer via efficient exploration of the possible space. ChemReasoner uses prior probabilities that could be derived from a LLM to initiate the exploration, and guides it via a reward obtained from the exploration process to prune unpromising actions. We currently
use “adsorption energy”, a key measure of reactivity as the reward function.}
\label{fig:challenge_and_approach}
\end{figure*}

Our works is aimed at enabling natural language question-answering capabilities to discover the best catalysts for a given chemical reaction.  Determining the best catalyst for a given reaction is a multi-step process. The first step involves combinatorial reasoning by finding an optimal set of descriptors that identify a catalyst. Formally, given a question which has relevant chemical properties $\mathbf{P},|\mathbf{P}|=n$ (e.g. ``crystal planes", ``porosity") and we want to identify the optimal subset $\mathbf{R\subset \mathbf{P}},|\mathbf{R}|=r$ for the language model to reason about. Considering that language models are sensitive to input permutations, there are $P^{n}_{r}=\frac{n!}{(n-r)!}$ possible prompt combinations. This goal can be accomplished by learning to prompt the LLM with the most relevant subset of properties \cite{deng-etal-2022-rlprompt} or decomposing the set into a sequence of chained queries \cite{dohan2022language} or a tree-structured space of queries \cite{sprueill2023monte}. In all cases, identification of the prompt-generating property subset becomes the limiting factor. 

Once a potential candidate is identified inside an LLM-driven reasoning step, evaluating the goodness of the catalyst is important for ranking or pruning the search.  For simple reactions, the goodness of a catalyst can be evaluated by the adsorption energy function of the chemical structure that reflects the amount of external energy required to drive a successful interaction between the catalyst and the reactant, and form a stable product. Generally, catalysts with lower adsorption energy are preferred since they would enable chemical reactions with lower energy requirements.  However, for complex reactions, the interaction between the catalyst and the reactant leads to formation of intermediate chemical structures, which further react between themselves and the catalyst to form the final output from the reaction. Each of the possible outcomes are defined as a ``reaction pathway".  Beginning with the same reactant or even the same intermediate products, a reaction can pursue different pathway depending on the orientation and stability of an intermediate product.  Therefore, for complex reactions, evaluating catalysts solely based on adsorption energy is not enough and considering energy requirements for enabling intermediate steps, and steering the reaction with high likelihood (also known as ``selectivity") towards a preferred pathway becomes an  important consideration.  Traditionally, properties such as adsorption energy, or selectivity to measure the goodness of a catalyst candidate are determined by spatial or structure-based reasoning methods building on computational chemistry principles.  

Our work combines these two steps by guiding the LLM-driven heuristic search guided via feedback from structure-driven reasoning methods trained from quantum chemistry simulations (Figure \ref{fig:challenge_and_approach}).  The heuristic search is implemented to emulate a screening mechanism where newer constraints are added in an iterative fashion. Candidates generated by the LLM are then transformed into a 3D atomistic representation involving the catalyst and the reactant. Such methods consider relative orientation of chemical structures in a 3D space, probabilistic consideration of reaction pathways involving intermediate chemical structures, and factoring in molecular dynamics to evaluate the stability of a given reaction pathway. In short, reasoning about complex scientific phenomenon is compositional and involves methodologies that the first-generation of LLMs are not trained with.


% In this work, we focus on the problem of suggesting the top-$k$ catalysts for a given chemical reaction and generating the reasoning for each candidate. In collaboration with researchers from the catalysis community, we developed a new dataset, BioFuels Question Reasoning dataset, of complex reasoning questions and answers \carl{we should discuss our relation to that work here and describe this as a more comprehensive study?} \carl{cite anonymized work}.  We observe the reasoning pathways used by domain scientists and conclude that it is important for LLMs to progress from ``thinking step-by-step'' to ``thinking step-by-step in terms of relevant properties''. 

 To solve this problem, we propose a generic methodology that makes two contributions. 1) It addresses the combinatorial challenge of query decomposition, and 2) brings in a chemistry-aware ML component to improve the fidelity of the resultant system. Considering the practical challenges of learning prompts that are both human comprehensible (a key consideration for scientists) and provide the best performance \cite{deng-etal-2022-rlprompt}, we pursue a stochastic, heuristic search-based approach that leverages LLMs trained on scientific literature with sophisticated instruction following capabilities \cite{ouyang2022training}. We formulate the task as a search problem in which an agent performs a query in an uncertain environment (represented by the LLM) and determines a query variant to pursue based on the perceived reward.  The search initially begins guided by prior probabilities that are obtained from LLM-derived representations and is subsequently guided by feedback from a scoring function that represents the goodness of catalysts found by the LLM-search (Figure \ref{eq:policy}.  Estimation of the energy of a chemical structure is at the core of developing efficient chemical reactions.  Finding catalysts that can enable chemical reactions with the least amount of external energy is key to developing environmentally friendly industrial processes. Therefore, we use the energy function of the stable configuration of catalyst-adsorbate combination as the guiding scoring or reward function.

% \carl{I think we need a ``why do I care about catalysis'' paragraph somewhere in the introduction here.}
 
 % \heng{define reward, and what it's used for} 

%Our second major contribution in this paper comes from demonstrating the value of a scientific domain-specific reward function into LLM-based computations.  Estimation of the energy of a chemical structure is at the core of developing efficient chemical reactions (see section \ref{sec:motivation_energy_func} for details).  Finding catalysts that can enable chemical reactions with least amount of external energy is key to developing environmentally friendly industrial processes. In this work, we implement such energy function specific considerations via a LLM-derived reward function.  Our experiments (using questions detailed in Table \ref{fig:qa_table_biofuels}) show that a simplistic integration of such a fundamental scientific concept dramatically improves the specificity of answers and their associated reasoning  

\noindent In summary, we make the following contributions:
\begin{enumerate}[leftmargin=*]
\itemsep-0.3em 
    \item We introduce \name: a novel hypothesis generation and testing framework that brings together LLM-driven heuristic search with quantum chemistry-guided feedback to enable natural language-based catalyst search and reasoning.
    \item Introduction of an automated planning step outperforms a search implemented based on descriptors provided by domain experts.
    % prompt strategy generation for LLM-driven complex scientific reasoning tasks as a stochastic search problem in an uncertain environment and propose a Monte Carlo Tree Search-based approach.
    \item We provide quantitative and qualitative demonstrations that the ``domain-grounding of LLMs" via quantum chemical property feedback leads to significant improvement over pure LLM-based implementations.
    \item We demonstrate that introduction of LLM-derived priors leads to efficient exploration of the chemical space that is also semantically coherent and explainable to end-users.
    \item We are first to consider reaction-pathway based reasoning.
    \item \carl{explainability contribution??}

\end{enumerate}

% \textcolor{red}{In contribution: ``we perform in-depth qualitative analysis from expert researchers in a scientific field with a high barrier for analysis.'' needs rewording}
 
  % focus on finding novel Given each query and its answers, we execute a reward function to rank potential answers.  For example, given a target chemical compound, the amount of external energy expended for its production is a measure of its desirability and of the process used to produce it.  Such measures can be computed by a language model either through a prompt or via delegation to an external function.  Assuming the reward surface is smooth as we construct and navigate the tree, our stochastic tree search systematically explores the query space and returns the best possible answer.

% Returning to our focus into chemistry-specific challenges, answering a question such as finding top-K catalysts for a given reaction and specific conditions requires reasoning about different factors. Additionally, for such answers to drive scientific hypothesis generation and inspire further consideration, scientists prefer answers that are grounded in specific technical concepts over simplified answers that could gleaned from general purpose resources such as Wikipedia (see Fig. TBD).  In terms of querying a LLM, such results can be achieved either through prompting the LLM with most relevant subset of scientific concepts, or decomposing the set into a sequence of chained-queries \cite{dohan2022language}.  In either way, identification of the prompt-generating subset becomes the limiting factor.  





% We formally define such queries as follows: 1) an initial specification of the problem (hereby described as a ``base query”) and 2) ``actions” that further constrain the query, and 3) an evaluation function that ranks candidate answers.   We posit that the language model can implicitly make the logical associations between the specified constraints and does not require explicit specification such as a database or knowledge graph query.  

% Our work is motivated by prior research that demonstrates that the most efficient prompts may not be human readable.  Therefore, seeking to generate most human-interpretable queries may further require alignment between logical representation of a scientific domain and the language model’s internal representation of said knowledge.   




% The sensitivity of language models to their input has triggered much research on learning and designing effective prompts \cite{deng-etal-2022-rlprompt}.  Approaches such as chain-of-thought (CoT) prompting \cite{kojima2022large} have became popular for generating responses with reasoning, especially for models trained with human feedback.  Much of the research in this area has focused on arithmetic reasoning, in which a mathematical task is solved in a step-by-step fashion~\cite{wei2022chain, reversecot2023}.  Given a specific task, reinforcement learning with human feedback (RLHF) methods and CoT variants \cite{zelikman2022star} collectively focus on improving the answer accuracy as well as reasoning.  The methods demonstrate that prompts that invoke reasoning not only improve the explainability of the language model output, but also lead to improvement in the answer accuracy itself.  Going beyond RLHF and CoT methods, it has also been shown that decomposition of a complex question into a sequence of tasks, or query decomposition, leads to further improvement in model performance \cite{creswell2022faithful, creswell2022selection, dohan2022language, jung2022maieutic, zhou2022least, wang2022self, yao2023tree}.

% \heng{elaborate why this is a challenging problem? how big is the search space? and why LLMs can help?}
% \heng{here needs a transition sentence, say we are using XXX problem in the chemical area as a case study.}
% \sutanay{Leaving Heng's questions to see how they have been addressed.}





  % Another related topic in this context is the non-deterministic aspect of querying language models.  The same question posed to the language model can elicit different answers and the variations increase with the complexity and size of query context.  If the environment is stochastic there is an inevitable uncertainty in the model’s predictions.







% Many scientific fields such as chemistry are highly empirical.  For example, discovering new catalysts is key to breakthroughs in designing the energy efficient chemical processes, and in past such discovery has largely followed an experiment-driven path.  Many scientific fields such as catalysis do not have a massive amount of observational data, which has limited potential for big data-driven machine-learning tools.  For them selective experiment design is crucial for minimizing costs and delays to key results.  However, experiment design is an art that strongly depends on a researcher’s knowledge of the extensive literature and ability to reason about promising hypotheses.  Large language models trained from scientific literature can be particularly impactful for such ideation and hypothesis generation.  In this work, we focus on the catalyst recommendation problem: given a set of reactants, an initial candidate catalyst and operating conditions such as pressure and temperature, what are the most optimal catalysts to recommend? 



% For example, Figure 1a shows an example response from GPT-3.5. However, we can execute the same query repeatedly with varied random seeds and obtain different answers.  Figure 1b shows a distribution of candidate catalysts from $N$-execution of the query.  In short, this illustrates a class of reasoning queries where we need to explore the space of possible queries and answers, and produce a list of ranked candidates, each accompanied by different ``chain-of-thoughts".  Finally, Figure 1c shows how this query space can be explored via two dimensions.  We can generate specialized queries and progressively generate narrower candidate spaces by considering more scientific concepts.  Given a set of scientific concepts, we can also generate multiple query variants with different semantic interpretations. \heng{here need to define what are queries and answers}


==> iclr2024-latex/backup/results.tex <==
\section{Experiments}

\begin{table}[tbp]
\centering
\caption{TBD}
\vspace{-0.5em}
    % \resizebox{0.5\textwidth}{!}{ 
\begin{tabular}{p{3.5em}|cc|cc}
    \hline
 &\multicolumn{2}{c|}{\textbf{OpenCatalysis}}&\multicolumn{2}{c|}{\textbf{BioFuels}}\\\hline
Method & Reward & $N_q $& Reward & $N_q$\\\hline\hline
CoT & 2.04 & 2 & 2.23 & 4.\\\hline
Sampling & 3.43 & 20. & 6.41 & 31.\\\hline
ToT & 9.91 & 505.8 & TBD & TBD\\\hline
MCR & 12.47 & 601.8 & 13.77 & 950.5\\\hline\hline
\end{tabular}
% }
\label{tab:multi-relation}
\vspace{-0.5em}
\end{table}

In this section, we present evaluation of $\ourSystem$'s performance across queries representing diversity in chemical reactions as well varying the reasoning complexity.  We also perform a qualitative evaluation of $\ourSystem$'s outputs through rigorous evaluation by researchers specialized in catalysis design.
% \carl{There's a lot of sections here which we probably don't want for a short paper due to space. (each 5.4.1 etc. takes up a line) }

\textbf{Datasets} We conduct our experiments on two catalysis datasets. The first one is curated from the OC20 \cite{chanussot2010open} and OC22 \cite{tran2023open} datasets published by the OpenCatalysis project \cite{zitnick2020introduction}.  The second one is a newly developed dataset with complex reasoning queries focused on biofuels-focused catalyst discovery.  Please see section \ref{sec:datasets} for details on these datasets.  We will release both these datasets upon acceptance of the paper.

\textbf{Baselines} We benchmark $\ourSystem$'s performance with three recent methods: 1) Chain-Of-Thought (CoT) prompting \cite{kojima2022large}, 2) an adaptation of Self-consistency based CoT \cite{wang2022self}, 3) breadth-first-search based Tree-of-Thoughts \cite{yao2023tree}.  
We did not include the depth-first-search method from Tree-of-Thoughts because our search does not have a clear ending criterion.  All our experiments are based on the GPT-3.5 text-davinci-003 model.  Our preliminary evaluations included Galactica \cite{taylor2022galactica} models with 6.7B and 30B parameters.  However, it's responses to chain-of-thought queries with instruction following (to generate list of candidates and then invoking the reward function computation over the returned list) lacked consistency to meet query chaining needs with $\ourSystem$.

% \subsection{Baselines \carl{This should probably be in appendix. We can refer the reader there. Also need to add citations.}}
% We evaluate $\ourSystem$'s performance with the following language models: (can try Galactica \carl{remove this}), GPT-3.5, (also trying GPT-4).
% \begin{enumerate}
%     \item \textsl{Single-Shot Query}: For each of these language models, we execute a query and parse the answer $A$ (such as a recommended catalyst) from the model generated response.  We return a pair ($A$, reward($A$)) as the answer. 
%     \item \textsl{Single-Shot Query with CoT prompt}: For each of these language models, we execute a query and parse the answer $A$ (such as a recommended catalyst) from the model generated response.  We return a pair ($A$, reward($A$)) as the answer. 
%     \item \textsl{Most Frequent Answer}: Given a language model, we execute the same query $N$ times following the above process.  Given this answer set $A_N$, we return a pair ($A_f$, reward($A_f$)) as the answer, where $A_f$ is the most frequently occurring answer in $A_N$.
%     \item \textsl{Most Frequent Answer with CoT prompt}: Given a language model, we execute the same query $N$ times following above process.  Given this answer set $A_N$, we return a pair ($A_f$, reward($A_f$)) as the answer, where $A_f$ is the most frequently occurring answer in $A_N$.
%     \item Comparison with BFS and DFS implementation (used in the Tree-of-Thought paper).
% \end{enumerate}

% \subsection{Metrics \carl{Probably want most of this in the appendix, although I'm not sure we are using these metrics anymore anyway?}}
% \textbf{Reward ratio}: Given a query $Q$, reward function $f_R(\cdot)$ we compare the rewards across a baseline method $M$ and $\ourSystem$ by computing the ratio $f_R(MCR(Q))/f_R(M(Q))$.

% \begin{table}
%     \centering
%     \caption{Caption for table \carl{Add column for # acerage API calls. Possibly column with results for OpenCatalysis}}
%     {\begin{tabular}{ccc}
%     &\bf{OpenCatalysis} & \bf{BioFuels}\\
%     Single Shot&2.04&2.23\\
%     Multi Shot&3.43&6.410833\\
%     BFS&9.91&\\
%     MCR&12.47&13.765
%     \end{tabular}}
%     \label{tab:settings}
% \end{table}





% \begin{table}
%     \centering
%     \caption{Caption for table \carl{Add column for # acerage API calls. Possibly column with results for OpenCatalysis}}
%     {\begin{tabular}{ccc}
%     &\bf{OpenCatalysis} & \bf{BioFuels}\\
%     Single Shot&2.04&2.23\\
%     Multi Shot&3.43&6.410833\\
%     BFS&9.91&\\
%     MCR&12.47&13.765
%     \end{tabular}}
%     \label{tab:settings}
% \end{table}

% \textbf{Precision and MRR}: Alternatively, if the domain experts provide us with a correct or preferred answer for each query AND if we could retrieve a list from all querying methods then we can also compute the precision/recall and mean reciprocal rank (MRR).  

% Precision = Number of queries in which a query answer contains correct answer/Number of Queries

% If our method/all methods return a list, then MRR would capture where the correct answer falls in the list.  Methods that rank the correct answer higher in its answer list would get a higher score.

\heng{define reward function formally}



\subsection{Qualitative Analysis Against Expert Reasoning}

\begin{figure}[!h]
  \centering
  \includegraphics[width=0.48\textwidth]{emnlp2023-latex/figures/eval-tree-depth-cost.png}
\caption{Illustration of an evaluation by a domain expert on the progression of top search results found on the path to the answer with highest reward.}
\label{fig:eval-1-mcr}
\end{figure}

\begin{figure*}[!h]
  \centering
  \includegraphics[width=1.0\textwidth]{emnlp2023-latex/figures/eval-1-qa.png}
\caption{Example question and human answer from our compiled QA-dataset.}
\label{fig:eval-1-qa}
\end{figure*}

\begin{figure*}[!h]
  \centering
  \includegraphics[width=1.0\textwidth]{emnlp2023-latex/figures/eval-1-gpt-3.5.png}
\caption{Response to above query returned by GPT-3.5.}
\label{fig:eval-1-gpt-3}
\end{figure*}

\begin{figure*}[!h]
  \centering
  \includegraphics[width=1.0\textwidth]{emnlp2023-latex/figures/eval-1-mcr.png}
\caption{Response to above query returned by MCR.}
\label{fig:eval-1-mcr}
\end{figure*}

\begin{figure*}[!h]
  \centering
  \includegraphics[width=0.5\textwidth]{emnlp2023-latex/figures/eval-1-comp.png}
\caption{Comparison of MCR vs GPT-3.5 by domain expert.}
\label{fig:eval-1-mcr}
\end{figure*}



\begin{figure*}[!h]
  \centering
  \includegraphics[width=0.6\textwidth]{emnlp2023-latex/figures/eval-tree-depth-no-cost.png}
\caption{Illustration of an evaluation by a domain expert on the progression of top search results found on the path to the answer with highest reward.}
\label{fig:eval-1-mcr}
\end{figure*}

\textcolor{blue}{Henry} Get output for 5 queries from the catalysis dataset (mcr, singleshot, singleshot frequent, bfs)

\textcolor{blue}{Sutanay} Compare answers with expert answer




==> iclr2024-latex/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

